A Verified Decision Procedure for Univariate Real Arithmetic with the BKR Algorithm

We formalize the univariate fragment of Ben-Or, Kozen, and Reif's (BKR) decision procedure for first-order real arithmetic in Isabelle/HOL. BKR's algorithm has good potential for parallelism and was designed to be used in practice. Its key insight is a clever recursive procedure that computes the set of all consistent sign assignments for an input set of univariate polynomials while carefully managing intermediate steps to avoid exponential blowup from naively enumerating all possible sign assignments (this insight is fundamental for both the univariate case and the general case). Our proof combines ideas from BKR and a follow-up work by Renegar that are well-suited for formalization. The resulting proof outline allows us to build substantially on Isabelle/HOL's libraries for algebra, analysis, and matrices. Our main extensions to existing libraries are also detailed.

==> arxivzip/arxivsnippets.tex <==
\snip{decideexistentialdef}{1}{2}{%
\isacommand{definition}\isamarkupfalse%
\ decide{\isacharunderscore}existential\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}rat\ poly\ fml\ {\isasymRightarrow}\ bool{\isachardoublequoteclose}\isanewline
\isakeyword{where}\ {\isachardoublequoteopen}decide{\isacharunderscore}existential\ fml\ {\isacharequal}\ {\isacharparenleft}let\ {\isacharparenleft}fml{\isacharunderscore}struct{\isacharcomma}polys{\isacharparenright}\ {\isacharequal}\ convert\ fml\ in\isanewline
\ \ find\ {\isacharparenleft}lookup{\isacharunderscore}sem\ fml{\isacharunderscore}struct{\isacharparenright}\ {\isacharparenleft}find{\isacharunderscore}consistent{\isacharunderscore}signs\ polys{\isacharparenright}\ {\isasymnoteq}\ None{\isacharparenright}{\isachardoublequoteclose}%
}%endsnip
\snip{decisionprocedurethm}{1}{2}{%
\isacommand{theorem}\isamarkupfalse%
\ decision{\isacharunderscore}procedure{\isacharcolon}\isanewline
\ {\isachardoublequoteopen}{\isacharparenleft}{\isasymforall}x{\isacharcolon}{\isacharcolon}real{\isachardot}\ fml{\isacharunderscore}sem\ fml\ x{\isacharparenright}\ {\isasymlongleftrightarrow}\ decide{\isacharunderscore}universal\ fml{\isachardoublequoteclose}\isanewline
\ {\isachardoublequoteopen}{\isacharparenleft}{\isasymexists}x{\isacharcolon}{\isacharcolon}real{\isachardot}\ fml{\isacharunderscore}sem\ fml\ x{\isacharparenright}\ {\isasymlongleftrightarrow}\ decide{\isacharunderscore}existential\ fml{\isachardoublequoteclose}%
}%endsnip
\snip{rootsdef}{1}{2}{%
\isacommand{definition}\isamarkupfalse%
\ roots\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}real\ poly\ {\isasymRightarrow}\ real\ set{\isachardoublequoteclose}\ \isakeyword{where}\ \isanewline
\ \ {\isachardoublequoteopen}roots\ p\ {\isacharequal}\ {\isacharbraceleft}x{\isachardot}\ poly\ p\ x\ {\isacharequal}\ {\isadigit{0}}{\isacharbraceright}{\isachardoublequoteclose}%
}%endsnip
\snip{consistentsignsatrootsdef}{1}{2}{%
\isacommand{definition}\isamarkupfalse%
\ consistent{\isacharunderscore}signs{\isacharunderscore}at{\isacharunderscore}roots\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}real\ poly\ {\isasymRightarrow}\ real\ poly\ list\ {\isasymRightarrow}\ \isanewline
\ \ rat\ list\ set{\isachardoublequoteclose}\isanewline
\isakeyword{where}\ {\isachardoublequoteopen}consistent{\isacharunderscore}signs{\isacharunderscore}at{\isacharunderscore}roots\ p\ qs\ {\isacharequal}\ {\isacharparenleft}sgn{\isacharunderscore}vec\ qs{\isacharparenright}\ {\isacharbackquote}\ {\isacharparenleft}roots\ p{\isacharparenright}{\isachardoublequoteclose}%
}%endsnip
\snip{matrixequationthm}{1}{2}{%
\isacommand{theorem}\isamarkupfalse%
\ matrix{\isacharunderscore}equation{\isacharcolon}\isanewline
\isakeyword{assumes}\ {\isachardoublequoteopen}p{\isasymnoteq}{\isadigit{0}}{\isachardoublequoteclose}\isanewline
\isakeyword{assumes}\ {\isachardoublequoteopen}{\isasymAnd}q{\isachardot}\ q\ {\isasymin}\ set\ qs\ {\isasymLongrightarrow}\ coprime\ p\ q{\isachardoublequoteclose}\isanewline
\isakeyword{assumes}\ {\isachardoublequoteopen}distinct\ signs{\isachardoublequoteclose}\isanewline
\isakeyword{assumes}\ {\isachardoublequoteopen}consistent{\isacharunderscore}signs{\isacharunderscore}at{\isacharunderscore}roots\ p\ qs\ {\isasymsubseteq}\ set\ signs{\isachardoublequoteclose}\isanewline
\isakeyword{assumes}\ {\isachardoublequoteopen}{\isasymAnd}l\ i{\isachardot}\ l\ {\isasymin}\ set\ subsets\ {\isasymLongrightarrow}\ i\ {\isasymin}\ set\ l\ {\isasymLongrightarrow}\ i\ {\isacharless}\ length\ qs{\isachardoublequoteclose}\isanewline
\isakeyword{shows}\ {\isachardoublequoteopen}M{\isacharunderscore}mat\ signs\ subsets\ {\isacharasterisk}\isactrlsub v\ w{\isacharunderscore}vec\ p\ qs\ signs\ {\isacharequal}\ v{\isacharunderscore}vec\ p\ qs\ subsets{\isachardoublequoteclose}%
}%endsnip
\snip{findconsistentsignsatrootsthm}{1}{2}{%
\isacommand{theorem}\isamarkupfalse%
\ find{\isacharunderscore}consistent{\isacharunderscore}signs{\isacharunderscore}at{\isacharunderscore}roots{\isacharcolon}\isanewline
\isakeyword{assumes}\ {\isachardoublequoteopen}p\ {\isasymnoteq}\ {\isadigit{0}}{\isachardoublequoteclose}\isanewline
\isakeyword{assumes}\ {\isachardoublequoteopen}{\isasymAnd}q{\isachardot}\ q\ {\isasymin}\ set\ qs\ {\isasymLongrightarrow}\ coprime\ p\ q{\isachardoublequoteclose}\isanewline
\isakeyword{shows}\ {\isachardoublequoteopen}set\ {\isacharparenleft}find{\isacharunderscore}consistent{\isacharunderscore}signs{\isacharunderscore}at{\isacharunderscore}roots\ p\ qs{\isacharparenright}\ {\isacharequal}\ \isanewline
\ \ consistent{\isacharunderscore}signs{\isacharunderscore}at{\isacharunderscore}roots\ p\ qs{\isachardoublequoteclose}%
}%endsnip
\snip{calcdatadef}{1}{2}{%
\isacommand{fun}\isamarkupfalse%
\ calc{\isacharunderscore}data\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}real\ poly\ {\isasymRightarrow}\ real\ poly\ list\ {\isasymRightarrow}\ \isanewline
\ \ {\isacharparenleft}rat\ mat\ {\isasymtimes}\ {\isacharparenleft}nat\ list\ list\ {\isasymtimes}\ rat\ list\ list{\isacharparenright}{\isacharparenright}{\isachardoublequoteclose}\isanewline
\isakeyword{where}\ {\isachardoublequoteopen}calc{\isacharunderscore}data\ p\ qs\ {\isacharequal}\ {\isacharparenleft}let\ len\ {\isacharequal}\ length\ qs\ in\isanewline
if\ len\ {\isacharequal}\ {\isadigit{0}}\ then\isanewline
\ \ {\isacharparenleft}{\isasymlambda}{\isacharparenleft}a{\isacharcomma}b{\isacharcomma}c{\isacharparenright}{\isachardot}{\isacharparenleft}a{\isacharcomma}b{\isacharcomma}map\ {\isacharparenleft}drop\ {\isadigit{1}}{\isacharparenright}\ c{\isacharparenright}{\isacharparenright}\ {\isacharparenleft}reduce{\isacharunderscore}system\ p\ {\isacharparenleft}{\isacharbrackleft}{\isadigit{1}}{\isacharbrackright}{\isacharcomma}base{\isacharunderscore}case{\isacharunderscore}info{\isacharparenright}{\isacharparenright}\isanewline
else\ if\ len\ {\isasymle}\ {\isadigit{1}}\ then\ reduce{\isacharunderscore}system\ p\ {\isacharparenleft}qs{\isacharcomma}base{\isacharunderscore}case{\isacharunderscore}info{\isacharparenright}\isanewline
else\ {\isacharparenleft}let\ qs{\isadigit{1}}\ {\isacharequal}\ take\ {\isacharparenleft}len\ div\ {\isadigit{2}}{\isacharparenright}\ qs{\isacharsemicolon}\ left\ {\isacharequal}\ calc{\isacharunderscore}data\ p\ qs{\isadigit{1}}{\isacharsemicolon}\isanewline
\ \ \ \ \ \ \ \ \ \ qs{\isadigit{2}}\ {\isacharequal}\ drop\ {\isacharparenleft}len\ div\ {\isadigit{2}}{\isacharparenright}\ qs{\isacharsemicolon}\ right\ {\isacharequal}\ calc{\isacharunderscore}data\ p\ qs{\isadigit{2}}\ in\isanewline
\ \ \ \ \ \ \ \ reduce{\isacharunderscore}system\ p\ {\isacharparenleft}combine{\isacharunderscore}systems\ p\ {\isacharparenleft}qs{\isadigit{1}}{\isacharcomma}left{\isacharparenright}\ {\isacharparenleft}qs{\isadigit{2}}{\isacharcomma}right{\isacharparenright}{\isacharparenright}{\isacharparenright}{\isacharparenright}{\isachardoublequoteclose}%
}%endsnip
\snip{findconsistentsignsatrootsdef}{1}{2}{%
\isacommand{definition}\isamarkupfalse%
\ find{\isacharunderscore}consistent{\isacharunderscore}signs{\isacharunderscore}at{\isacharunderscore}roots\ {\isacharcolon}{\isacharcolon}\isanewline
\ {\isachardoublequoteopen}real\ poly\ {\isasymRightarrow}\ real\ poly\ list\ {\isasymRightarrow}\ rat\ list\ list{\isachardoublequoteclose}\isanewline
\ \isakeyword{where}\ {\isachardoublequoteopen}find{\isacharunderscore}consistent{\isacharunderscore}signs{\isacharunderscore}at{\isacharunderscore}roots\ p\ qs\ {\isacharequal}\ \isanewline
\ \ {\isacharparenleft}let\ {\isacharparenleft}M{\isacharcomma}S{\isacharcomma}{\isasymSigma}{\isacharparenright}\ {\isacharequal}\ calc{\isacharunderscore}data\ p\ qs\ in\ {\isasymSigma}{\isacharparenright}{\isachardoublequoteclose}%
}%endsnip
\snip{kroneckerproductdef}{1}{2}{%
\isacommand{definition}\isamarkupfalse%
\ kronecker{\isacharunderscore}product\ {\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}{\isacharprime}a\ {\isacharcolon}{\isacharcolon}\ ring\ mat\ {\isasymRightarrow}\ {\isacharprime}a\ mat\ {\isasymRightarrow}\ {\isacharprime}a\ mat{\isachardoublequoteclose}\isanewline
\isakeyword{where}\ {\isachardoublequoteopen}kronecker{\isacharunderscore}product\ A\ B\ {\isacharequal}\ {\isacharparenleft}\isanewline
let\ ra\ {\isacharequal}\ dim{\isacharunderscore}row\ A{\isacharsemicolon}\ ca\ {\isacharequal}\ dim{\isacharunderscore}col\ A{\isacharsemicolon}\ rb\ {\isacharequal}\ dim{\isacharunderscore}row\ B{\isacharsemicolon}\ cb\ {\isacharequal}\ dim{\isacharunderscore}col\ B\ in\isanewline
\ \ mat\ {\isacharparenleft}ra\ {\isacharasterisk}\ rb{\isacharparenright}\ {\isacharparenleft}ca\ {\isacharasterisk}\ cb{\isacharparenright}\isanewline
\ \ \ \ {\isacharparenleft}{\isasymlambda}{\isacharparenleft}i{\isacharcomma}j{\isacharparenright}{\isachardot}\ A\ {\isachardollar}{\isachardollar}\ {\isacharparenleft}i\ div\ rb{\isacharcomma}\ j\ div\ cb{\isacharparenright}\ {\isacharasterisk}\ B\ {\isachardollar}{\isachardollar}\ {\isacharparenleft}i\ mod\ rb{\isacharcomma}\ j\ mod\ cb{\isacharparenright}{\isacharparenright}{\isacharparenright}{\isachardoublequoteclose}%
}%endsnip
\snip{rowstokeepdef}{1}{2}{%
\isacommand{definition}\isamarkupfalse%
\ rows{\isacharunderscore}to{\isacharunderscore}keep{\isacharcolon}{\isacharcolon}\ {\isachardoublequoteopen}{\isacharparenleft}{\isacharprime}a{\isacharcolon}{\isacharcolon}field{\isacharparenright}\ mat\ {\isasymRightarrow}\ nat\ list{\isachardoublequoteclose}\isanewline
\ \ \isakeyword{where}\ {\isachardoublequoteopen}rows{\isacharunderscore}to{\isacharunderscore}keep\ A\ {\isacharequal}\ map\ snd\ {\isacharparenleft}pivot{\isacharunderscore}positions\ \isanewline
\ \ {\isacharparenleft}gauss{\isacharunderscore}jordan{\isacharunderscore}single\ {\isacharparenleft}A\isactrlsup T{\isacharparenright}{\isacharparenright}{\isacharparenright}{\isachardoublequoteclose}%
}%endsnip
\snip{rowstokeepranklem}{1}{2}{%
\isacommand{lemma}\isamarkupfalse%
\ rows{\isacharunderscore}to{\isacharunderscore}keep{\isacharunderscore}rank{\isacharcolon}\isanewline
\isakeyword{assumes}\ {\isachardoublequoteopen}dim{\isacharunderscore}col\ A\ {\isasymle}\ dim{\isacharunderscore}row\ A{\isachardoublequoteclose}\isanewline
\isakeyword{shows}\ {\isachardoublequoteopen}vec{\isacharunderscore}space{\isachardot}rank\ {\isacharparenleft}length\ {\isacharparenleft}rows{\isacharunderscore}to{\isacharunderscore}keep\ A{\isacharparenright}{\isacharparenright}\ {\isacharparenleft}take{\isacharunderscore}rows\ A\ \isanewline
\ \ {\isacharparenleft}rows{\isacharunderscore}to{\isacharunderscore}keep\ A{\isacharparenright}{\isacharparenright}\ {\isacharequal}\ vec{\isacharunderscore}space{\isachardot}rank\ {\isacharparenleft}dim{\isacharunderscore}row\ A{\isacharparenright}\ A{\isachardoublequoteclose}%
}%endsnip
\snip{transposeranklem}{1}{2}{%
\isacommand{lemma}\isamarkupfalse%
\ transpose{\isacharunderscore}rank{\isacharcolon}\isanewline
\isakeyword{shows}\ {\isachardoublequoteopen}vec{\isacharunderscore}space{\isachardot}rank\ {\isacharparenleft}dim{\isacharunderscore}row\ A{\isacharparenright}\ A\ {\isacharequal}\ vec{\isacharunderscore}space{\isachardot}rank\ {\isacharparenleft}dim{\isacharunderscore}col\ A{\isacharparenright}\ {\isacharparenleft}A\isactrlsup T{\isacharparenright}{\isachardoublequoteclose}%
}%endsnip

